Autoencoders for unsupervised anomaly detection in high energy physics

Autoencoders are widely used in machine learning applications, in particular for anomaly detection. Hence, they have been introduced in high energy physics as a promising tool for model-independent new physics searches. We scrutinize the usage of autoencoders for unsupervised anomaly detection based on reconstruction loss to show their capabilities, but also their limitations. As a particle physics benchmark scenario, we study the tagging of top jet images in a background of QCD jet images. Although we reproduce the positive results from the literature, we show that the standard autoencoder setup cannot be considered as a model-independent anomaly tagger by inverting the task: due to the sparsity and the specific structure of the jet images, the autoencoder fails to tag QCD jets if it is trained on top jets even in a semi-supervised setup. Since the same autoencoder architecture can be a good tagger for a specific example of an anomaly and a bad tagger for a different example, we suggest improved performance measures for the task of model-independent anomaly detection. We also improve the capability of the autoencoder to learn non-trivial features of the jet images, such that it is able to achieve both top jet tagging and the inverse task of QCD jet tagging with the same setup. However, we want to stress that a truly model-independent and powerful autoencoder-based unsupervised jet tagger still needs to be developed.

==> framework.tex <==
\subsection{Jet data and autoencoder architecture}
\label{sec:framework}

\AlMu{I decided to only keep only the very essentials and move more all details to an appendix. There we should really give all details necessary for reproducibility. Probably, this section should become a subsection of the next one.} \AlMo{moved it up}

We consider binary classification, where the two classes are often called background and signal/anomaly, respectively, according to the physics context. We use a semisupervised setup where we assume that a data set consisting only of background data is available. For the main part of this work, we use top tagging as an example which is a well established benchmark in collider physics: Simulated QCD jets (initiated by light-flavour quarks or gluons) have to be distinguished from hadronically decaying boosted top-quarks which form single jets.
\par
For an easy comparison with the literature, we use the benchmark dataset from Ref.~\cite{Butter_2018}. \AlMu{Landscape of top taggers?} \TF{Changed to LoLa} A subset of 100K, 40K, and 40K jets of both types are used for the training, validation, and testing, respectively.
In the following, we describe our default setup which will be modified and improved in the next sections. We employ the preprocessing introduced in Ref.~\cite{Heimel_2019} \TF{Also wrong reference}\IO{I think the citation is actually correct as it seems to be the oldest source with the one to one equal preprocessing as we have. They do cite \cite{Macaluso_2018} that uses practically the same thing but with 37*37 grid and other eta and phi intervals.}. Hence, the jets are converted into two-dimensional jet images with $40\times40$ pixels. The details of the jet generation and the preprocessing are discussed in Appendix~\ref{sec:appendix}. Fig.~\ref{fig:average} shows the average images of both classes. For QCD jets, most of the intensity is concentrated in the central pixels. For top jets, there is a clearly visible 3 prong structure (as expected from a top-quark decay). Of course, individual jets are harder to distinguish than their average images may indicate.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/framework/average.png}
    \caption[Caption for LOF]{Average of 40K QCD (left) and top images (right) in the test set accoring to our preprocessing. \AlMu{Do $\eta$ and $\phi$ make sense as labels after we rotated the jets? In any case we should use $\Delta \eta$ and $\Delta \phi$?}}
    \label{fig:average}
\end{figure}

As our anomaly detection algorithm, we use a conventional convolutional autoencoder with an architecture similar to the one in Ref.~\cite{Kasieczka_2019}. Several convolution layers with $4\times 4$ kernel and average pooling layers with $2\times 2$ kernel are applied before the image is flattened and a fully connected network reduces the input further into the bottleneck latent space with 32 nodes. The described encoder structure is inverted to form the corresponding decoder which is used to reconstruct the original image from its latent space description. The architecture is sketched in Fig.~\ref{fig:AE3_arch} and described in full detail in Appendix~\ref{sec:appendix}. 
\par
The autoencoder is trained exclusively on the background data. To describe the goal of reconstructing the input image, again following the literature~\cite{Heimel_2019}, we use the mean squared error, i.e.\ the average of the squared error of each pixel with respect to its input value, as a loss function \TF{Check this}. During testing the value of the loss function is also used as the discriminator between signal and background. An event is tagged as signal/anomaly if the value of the loss function is larger than a given threshold. Changing the threshold value, one obtains the usual ROC curve.
\par
This procedure assumes that an unseen signal event cannot be reconstructed as well as a background event on which the autoencoder has been trained on. \IO{already discussed in introduction?} It is the main content of this work to investigate if and to what extent this assumption is valid.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/framework/AE3_arch.png}
    \caption[Caption for LOF]{Architecture of our autoencoder\footnotemark.}
    \label{fig:AE3_arch}
\end{figure}




==> preprocessing.tex <==
\label{sec:reproc}

\subsection{Motivation and method description} 
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.6\linewidth]{fig/nonzero.png}
%    \caption{Distribution of jet images in four categories (low $p_T$ and high $p_T$ QCD, top and DM), respective to the number of non-zero pixels.}
%    \label{fig:nonzero}
%\end{figure}
%
%Let us take a look at the distributions of jet images by the number of non-zero pixels in them represented in fig. \ref{fig:nonzero}. It makes it clear that the images generally have less than 100 pixels that contain jet constituents out of the total 1600 pixels. The examples of the random conventionally preprocessed jet images (see top left of \ref{fig:reproc} and first raw of fig.\ \ref{fig:examples}) not only show us that the images are sparse (consist of few non-zero pixels on a 0 background), but also that most non-zero pixels are much dimmer (have lower value) than the few bright ones. In the top right of fig. \ref{fig:reproc} we can see the distribution of the intensities of these pixels. The height of each bar on the plot shows the fraction of all non-zero pixels from 100,000 training top images with intensity in an interval on the x-axis (notice that the x-axis has a logarithmic scale). It can be seen, that this distribution is very uneven and most pixels are orders of magnitude dimer than the few bright ones. 
%\par
%%%%%Paragrph refering to AE
As shown in section \ref{sec:ignored}, bright pixels produce the most MSE loss in the image, and therefore the AE focuses on reconstructing them. On the contrary, it totally ignores the dim pixels as they are often not distinguishable from the 0 background in comparison with the bright ones at the beginning of the training. On the other hand, a lot of information can be stored in these dim regions. E.g.\ the dim region in the bottom right of the mentioned example image (fig. \ref{fig:reproc} and top left) may actually be the third sub-jet in the top jet structure. Unfortunately, it is not visible without highlighting and will most likely be ignored in the training of the AE. Our idea is to highlight these dim pixels, so the AE can learn the information and features stored in them. This way, the AE gets a chance to catch more distinctive features of the training set, and perform better at distinguishing anomalies.
\par
%%%%%Paragrph refering to AE/

This highlighting is done by applying a function $R : [0, 1]\rightarrow [0, 1]$ to the value of each pixel of the image created by the conventional preprocessing, thereby adjusting the distribution of the pixel intensities.
\par

\begin{figure}
    \begin{center}
        \includegraphics[width=0.5\textwidth]{fig/optional/rep_fkt.png}
    \end{center}
    \caption{Functions for alternative preprocessing.}
    \label{fig:rep_fct}
\end{figure}

The following functions are used for remapping the intensities: %alternative preprocessing:

\begin{itemize}
    \item $R0(x)=x$. This method does not change the initial image.
    \item $R1(x)=\sqrt{x}$. Motivation for this function is to compensate the discussed squaring of the error in MSE at the beginning of the AE training, which leads to the concentration on brightest pixels. 
    \item $R2(x)=\sqrt[4]{x}$
    \item $R3(x)=log(\alpha x+1)/log(\alpha+1)$ We arbitrarily took $\alpha=1000$.
    \item $R4(x)=\theta(x)$ where $\theta$ denotes the Heaviside function, therefore making all non-zero pixels of an image equal in intensity. 
\end{itemize}

The comparison plot of these functions is shown in fig \ref{fig:rep_fct}. \AlMo{despite what we said during the meetings I would keep this plot, people know what a square root looks like, but it is helpful to have this plot}
\par
After applying any of these functions the image is normalized once again, to have sum 1 (further we will always refer to the normalized images). Note that R1, R2 and R3 are monotone functions on $[0, 1]$ and therefore each has an inverse function. It means that by applying these functions we effectively lose no information about the distribution of the intensity in the image because the initial image can be restored. In contrast, R4 does not have an inverse function and leads to a significant distortion of the initial information. 
\par
On the left of fig. \ref{fig:reproc} images for the same top jet, but different preprocessing methods are shown. Instead of having a black picture with one (which is often the case by QCD and DM) or a few bright pixels that results from the preprocessing, we get an insight on a complex structure with many features. On the right of fig. \ref{fig:reproc} the distributions of intensities of non-zero pixels of 100,000 top images are shown. With conventional preprocessing, we get a strong disproportion of the intensities: the median (and so most of the pixels) of the distribution is more than a half order of magnitude away from the average value. As is illustrated on the lower subplots, the intensity remapping methods "squeeze" the distribution on the logarithmic scale. Distributions for R1 and R3, span across around 1.5 orders of magnitude, and the distribution for R2 lies nearly fully in one order of magnitude. The non-zero pixel intensities on one particular image after using R4 are all equal $1/$(Number of non-0 pixels in the image) because of the normalization, therefore we get different intensities for different pictures, and a narrow (on log scale) distribution instead of the delta function. We want to mention that these remappings do not change the number of non-0 pixels, and because of the normalization the average intensity of non zero pixels is unchanged. 
%\par
%\begin{equation}
%    \frac{\text{Sum of all image intensities}}{\text{Total number of non-zero pixels}}=\frac{1\cdot100000}{\text{Total number of non-zero pixels}}=const.
%\end{equation}
%
%It will remain constant after the transformation, which can also be seen on the distribution plots.

\AlMo{I would write the type of preprocessing already on the plots of 4.3 (so that it becomes more readable). Regarding the layout I would avoid referring to figures that are to many pages away (this is a thing that is corrected at the end anyway)}

\IO{Good idea with plot 4.1 I'll do that immediately. What plot is too far away you mean?}
\AlMo{Like in page 13 when you refer to fig. 4.3 and 4.4, but there's no point in correcting that now since there will be a major rewriting and rearrange}

\AlMo{I have moved those images even further away, I guess it would make sense to refer to some other image close by}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/preprocessing/reproc.png}
    \caption{Example of a top jet image (left), and the distribution of intensities of non-zero pixels for 100K top jet images (right) for different preprocessing methods from top to bottom R0, R1, R2, R3 and R4. Orange vertical lines on the distribution plots indicate the median of the distribution and the red dashed line indicates the average value of the distribution.}
    \label{fig:reproc}
\end{figure}



\subsection{Effects on the issues}


\subsubsection{Ignored pixels}
One of the main motivations to do the intensity remapping was to reduce the number of ignored pixels, so that more features of the image will be relevant for the reconstruction loss and hence there will be more features by which QCD and top jet images can be distinguished in such a manner. 
For a standard AE trained on normally preprocessed images the said histogram was shown in top of fig. \ref{fig:igno_pix}.  If we now train an AE on R2 preprocessed  images (see fig. \ref{fig:order_sp_QCD})  we see that now for QCD the AE reconstructs a total of 19.5\% of all pixels well compared to only about 13\% for the conventional (R0) preprocessing. Based on the peak of the average squared error curve we can now say that the AE now takes around 8 first pixels in consideration rather than around 4 for R0 case. Interestingly, we also observe that even less pixels are overreconstructed in this case. 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=1\linewidth]{fig/preprocessing/spectra_order_QCD_QCDR0R2.png}
%    \caption{Upper part: histograms of quality of reconstruction of non-0 pixels in QCD images by a AE trained on QCD images w.r.t. order of the pixel on the image when sorted in descending intensity order. Lower part: average true intensity and reconstructed intensity of the non-0 pixels mentioned above w.r.t. their order, and the average squared error of reconstruction of these pixels. Left: for R0 preprocessed images. Right: for R2 preprocessed images.}
%    \label{fig:order_sp_QCD}
%\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{fig/preprocessing/combinedignoR2.png}
    \caption{Upper part: histograms of quality of reconstruction of non-0 pixels in R" remapped images w.r.t. order of the pixel on the image when sorted in descending intensity order. Lower part: average true intensity and reconstructed intensity of the non-0 pixels mentioned above w.r.t. their order, and the average squared error of reconstruction of these pixels. Left: for QCD images. Right: for top images.}
    \label{fig:order_sp_QCD}
\end{figure}

Right of fig. \ref{fig:order_sp_QCD} shows the analogue plots for the case of training on the top jets. In this case the improvement is not that obvious. On one hand, the number of non-0 pixels in the 80\%-120\% of reconstruction intensity has increased from 9.33\% to 10.70\% of total. Also the minor increase is seen in 50\%-80\% interval, but the number of pixels with 10\%-50\% reconstruction (that can be considered as still not fully ignored) has decreased. The latter effect can be connected with the fact than AE does not always set the background around the intensive pixels to exactly 0 which could be enough to partially "reconstruct" the low intensity pixels that are situated around the high intensity ones for R0 case, but is absolutely not enough to give the pixels in second case a least 10\% of their intensity. From the lower plots we see that  before AE was only taking around 4 first pixels into account, when using R2 it considers 6-7 first pixels (based on the peak of the squared error curve).

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=1\linewidth]{fig/preprocessing/spectra_order_top_topR0R2.png}
%    \caption{Upper part: histograms of quality of reconstruction of non-0 pixels on a top images by a AE trained on top images w.r.t. order of the pixel on the image when sorted in descending intensity order. Lower part: average true intensity and reconstructed intensity of the non-0 pixels mentioned above w.r.t. their order, and the average squared error of reconstruction of these pixels. Left: for R0 preprocessed images. Right: for R2 preprocessed images.}
%    \label{fig:order_sp_top}
%\end{figure}

(MAYBE ADD A TABLE WITH THE PERCENTAGES OF IGNORED AND WELL RECONSTRUCTED)

\AlMo{Yes, I think making a table rather than mentioning all the percentages in the text would increase the overall clarity a lot}

\begin{table}
\centering
\begin{tabular}{c||c|c|c|c|c|c}
Reconstruction & $<$10\% & 10-20\% & 20-50 \% & 50-80 \% & 80-120\% &$>$120\%\\
\hline
\hline
QCD R0 & 58.74\% & 8.55 \% & 10.36 \% & 5.65 \% & 12.94 \% & 3.77 \% \\
QCD R2 & 54.26 \% & 11.39 \% & 8.61 \% & 4.63 \% & 19.52 \% & 1.59 \% \\
\hline
Top R0 & 45.91 \% & 14.04 \% & 17.75 \% & 7.34 \% & 9.33 \% & 5.64 \% \\
Top R2 & 55.01 \% & 12.29 \% & 11.49 \% & 8.32 \% & 10.70 \% & 2.19 \% \\
\hline
\end{tabular}
\caption{Percentage of pixels for a given reconstruction level}
\end{table}



\subsubsection{Correlations of loss with number of non-0 pixels}

In fig. \ref{fig:pixnum_MSE} we see the scatter plots of the loss of the test pictures against the number of non-zero pixels for R2 remapping and for direct and reverse tagging cases. 
\par
The lower row of fig. \ref{fig:pixnum_MSE} present the analogue scatter plots for the case of training and evaluation on the images preprocessed by the R2 (4-th root) method. We can see that this preprocessing have introduced a strong bias: images with less non-zero pixels produce more reconstruction loss. This bias works oppositely to the bias we have observed for R0. When we train on QCD the AE leans an efficient way to reconstruct these low pixel number images and therefore QCD will in general be better reconstructed than top, hence we get a direct tagger. If the training is done on the top images the AE has no possibility to learn on the low pixel numbers efficiently thus leaving the QCD images with low pixel numbers to be detected as the high loss anomalies, hence we get a reverse tagger. Low non-zero pixel number is a feature that is abundant in QCD set but is practically unseen in the top jets. By making it more loss rich (using our alternative preprocessing) we enabled the training of AE in the reverse direction. As we see from the right bottom figure for a range of around 20-40 pixels the top jets for each particular pixel number are now reconstructed a bit better than QCD (which is an improvement to the situation we see on the top right plot). Unfortunately, it is only valid for a small interval, and this difference is small compared to the width of the distribution or the slope of the bias. We see that most of the reverse tagging performance is based on the QCD images that have a too small number of pixels and therefore much higher loss compared to others (because of the new bias).

\begin{figure}[h]
\includegraphics[width = 0.5\textwidth]{fig/preprocessing/pixnum_loss_QCDR2.png}
\includegraphics[width = 0.5\textwidth]{fig/preprocessing/pixnum_loss_topR2.png}
\caption{Scatter plots of the losses versus number of non-zero pixels for all test images for R2 preprocessing. Left: AE trained on QCD. Right: AE trained on top. Solid lines show the avarage loss in each column.}
\label{fig:pixnum_MSE}
\end{figure}

\AlMo{If we decide to use correlation coefficient as measure we could define its change here}

If we look on fig. \ref{fig:dir_rev_top_MES} once more it looks as if the reverse tagger ROC curves converge to the limit of R4 preprocessing. We can plot the ROC curve for a tagger based on the non-0 pixel number distribution shown on fig. \ref{fig:nonzero}. One such tagger can be based on rule "signal (top jet images) are the images with the most nonzero pixels" that will give us a direct tagger of top jets that is plotted as an upper grey curve. We see that it performs significantly worse than the direct taggers for most of the remappings. If we now formulate the rule for a tagger as "top images are background and signal (QCD) are the images with the least number of non-0 pixels" we get (one of two possible) reverse taggers. This one is plotted on fig. \ref{fig:dir_rev_top_MES} as a lower puncture gray line that can be barely visible as it is overlaid from above with the dashed blue line of the R4 reverse tagger. The last named tagger has practically the same performance as this reverse pixel number tagger, and all other remappings give the ROC curves that are also very close to it. It shows once more that the reverse tagging for the alternative prepossessings relies on the correlation of loss with number of pixels on the plot. \AlMo{this discussion should be moved to net subsection and rather substituted by insight from the correlation plots on what that should mean for the tagging performance}


\subsection{Tagging performance}

The performances for direct and reverse taggers can be summarized by a fig. \ref{fig:dir_rev_top_MES} and table \ref{preproc_table}. The solid lines show the ROC curves of the direct tagger for different preprocessing cases. The dashed lines show the ROC curves of the reverse tagger (the tagger that is trained on top jets and is used to tag QCD jets as the ones that have higher losses). Bear in mind that for reverse tagger $\epsilon_S=\epsilon_{QCD}$ and $\epsilon_B=\epsilon_{top}$, so the lower the curves are the better is the QCD tagging performance of the reverse tagger. The ROC curve of the working reverse tagger must then be under the $\epsilon_{QCD}=\epsilon_{top}$ curve on this image. The AUC for both taggers is calculated for the curves on this plot with $\epsilon_{top}=y-axis$ and $\epsilon_{QCD}=x-axis$. The $AUC$ given on the plot is calculated for this particular with coordinates $\epsilon_B=\epsilon_{top}=x-axis$ and $\epsilon_S=\epsilon_{QCD}=y-axis$ plot although the conventional definition for the AUC of a tagger (given in table \ref{preproc_table}) is calculated for a reverse tagger from a plot with $\epsilon_B=\epsilon_{top}=y-axis$, $\epsilon_S=\epsilon_{QCD}=y-axis$ (an image mirrored along the diagonal). Therefore the conventional AUC for a reverse tagger equals $1-AUC$ of what is given in fig. \ref{fig:dir_rev_top_MES}.
%So the AUC for the reverse tagger is $1-AUC$ of it if the ROC curve would be plotted in the coordinate frame $\epsilon_B=\epsilon_{top}=x-axis$ $\epsilon_S=\epsilon_{QCD}=y-axis$ (mirroring along a diagonal) that is the standard method of describing AUC of a general tagger, therefore in the table with all the results the AUC of the reverse tagger is given in standard definition and therefore is equal to $1-AUC$ of mentioned value on the plot. The 
\par
The whole point of plotting both ROC in such a way is to see what change in $\epsilon_{QCD}$ and $\epsilon_{top}$ does training on different classes bring. The distance between ROC curves of direct and reverse tagging cases or difference between the the respective AUC values can be partially used as the measure of how flexible (unbiased) is a particular method. If we see no big difference as is in case of the R4 we can assume that there is some particularly strong bias that has en effect on losses of QCD and top jet images in such a way that the change in the loss due to the training on one or the other class is much smaller than the bias. We aim for a method that is as model independent and unbiased as possible, so both direct and reverse tagging are done well, therefore the distance between direct and reverse ROC curves is as large as possible. 
\par
As already discussed for the R0 preprocessing the direct tagger performs well, but although $\epsilon_{QCD}$ and $\epsilon_{top}$ change significantly for the reversed labels, the change is not enough to enable the true reverse tagging (still holds $\epsilon_{top}>\epsilon_{QCD}$, as such method is biased to reconstruct QCD generally better). In the R1 preprocessing case we have a minor decrease in the direct tagging performance, but a significant improvement in the reverse tagging performance so that the reverse tagging is now also possible. The further R2 and R3 preprocessings give strong decrease in direct tagging performance and the improvement in the reverse performance cases. The extreme R4 case the direct tagging becomes impossible, and the difference between the opposite learning processes is small, that denotes a possible strong bias in the model. 
For this particular dataset R1 seems to be optimal to nearly preserve the initial performance of the random tagger, but to also enable the reverse tagging.
\input{tables/preproc_table.tex}

%If the separation between two direct and reverse curves or the AUC values is large, it means that sort of the tagger we get after training depends more on the training than on the biases in the system. Hence we not only aim to find a method that would work in both direct and reverse case 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/roc/dir_rev/dir_rev_top_MSE_1x1.png}
    \caption{ROC curves of direct and reverse taggers trained on the images created using different prepossessing. The dotted show the ROC of the two taggers based on the number of the non-0 pixels on the image.}
    \label{fig:dir_rev_top_MES}
\end{figure}

ALTERNATIVELY
The performances for direct and reverse taggers can be summarized by a fig. \ref{fig:dir+rev_top_MSE}. The right sub figure shows that whereas an AE trained on top jets could not be considered a QCD tagger in the conventional case, it gets a significantly better performance than random tagger for quite ``soft'' R1 preprocessing (in comparison to R2, R3 and R4, which influence the non-zero pixel distribution even more). For other ``harder'' R2-R4 preprocessing AE performance is better and even reaches $AUC\approx0.7$. The left sub-figure shows that the performance of the direct tagger has a minor decrease for R1 preprocessing when compared to R0 case and quite strongly decrease of performance for R2 and R3 preprocessings but still much better than random tagger or pixel number based tagger (introduced further). For R4 the performance drops under the $\epsilon_S=\epsilon_B$ threshold of a random tagger. 

For this particular dataset R1 seems to be optimal to nearly preserve the initial performance of the random tagger, but to also eneble the reverse tagging.

\begin{figure}[h]
    \begin{minipage}{0.49\textwidth}
        \includegraphics[width=\linewidth]{fig/roc/dir/dir_top_MSE.png}
    \end{minipage}
    \begin{minipage}{0.49\textwidth}
        \includegraphics[width=\linewidth]{fig/roc/rev/rev_top_MSE.png}
    \end{minipage}
    \caption{Left: the ROC curves of the direct AE based taggers trained on the images done by different prepossessing. Right: the ROC curves of the reverse AE based taggers trained on the on the images done by different prepossessing. The dasched curve on both images is the $\epsilon_S=\epsilon_B$ curve, and the puncture curve shows the ROC curve for based on non-0 pixel numbers.}
    \label{fig:dir+rev_top_MSE}
\end{figure}
ADDITIONALLY
Fig. \ref{fig:dir_rev_DM_MES} shows the analogue ROC curves created for differently preprocessed images from the DM dataset.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=1\linewidth]{fig/roc/dir_rev/dir_rev_DM_MSE_1x1}
%    \caption{ROC curves of direct and reverse taggers trained on the images created using different prepossessing on a low $p_T$ QCD and DM sets. The dotted show the ROC of the two taggers based on the number of the non-0 pixels on the image.}
%    \label{fig:dir_rev_DM_MES}
%\end{figure}

\AlMo{we will need to eventually agree on how to present the ROC curves, I think showing direct and inverse on the same plot works best. Even more if we define a direct-inverse performance as the difference AUC(direct)-AUC(inverse) which corresponds to the area between the direct and inverse curve and in some sense evaluates how bidirectional our tagger is. So for instance for R1 we have 0.472, for R2 we have 0.424 and so on}

\AlMo{I hid the DM picture}

